Sig-DEG for Distillation: Making Diffusion Models Faster and Lighter

Diffusion models achieve state-of-the-art generative performance but remain computationally expensive at inference, often requiring many discretization steps. We propose Sig-DEG (Signature-based Differential Equation Generator), a generator for distilling pre-trained diffusion models. Inspired by high-order stochastic Taylor expansions, Sig-DEG combines partial signatures that summarize Brownian motion over subintervals with a recurrent structure to approximate stochastic differential equation solutions to achieve universality. We formulate distillation as supervised learning, matching fine-resolution teacher trajectories on a coarse time grid. At inference, Sig-DEG enables fast generation, as the partial signatures can be simulated exactly from their known distributions without requiring fine-grained Brownian paths. Experiments on image and time-series generation demonstrate competitive sample quality with inference speedups of up to several hundred times over the teacher. A Schr\"odinger bridge example further demonstrates Sig-DEG's applicability beyond diffusion distillation.

==> tables/rberg_T1500.tex <==
\begin{table}[ht]
  \centering
  \small
  \renewcommand{\arraystretch}{1.0}
  \setlength{\tabcolsep}{3pt}
  \caption{\textbf{rBerg} (1500-step teacher): Sig-DEG (SD) vs.\ CM at the same number of steps (mean $\pm$ standard deviation over 10 sampling runs of 20k samples; same protocol as Table~\ref{tab::rberg}).}
  \label{tab:rberg_T1500}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{rccccccc}
    \toprule
    & Teacher & \multicolumn{2}{c}{10 steps} & \multicolumn{2}{c}{5 steps} & \multicolumn{2}{c}{1 step} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
    Metric & (1500) & SD & CM & SD & CM & SD & CM \\
    \midrule
    Hist.\ $\downarrow$ & \pmc{0.0362}{0.0011} & \pmcb{0.0337}{0.0005} & \pmc{0.1261}{0.0013} & \pmcb{0.0337}{0.0008} & \pmc{0.1120}{0.0014} & \pmcb{0.0497}{0.0010} & \pmc{0.1204}{0.0011} \\
    CrossCorr $\downarrow$ & \pmc{0.1492}{0.0371} & \pmc{0.1238}{0.0108} & \pmcb{0.1198}{0.0150} & \pmcb{0.1035}{0.0166} & \pmc{0.1078}{0.0140} & \pmc{0.1256}{0.0039} & \pmcb{0.1207}{0.0139} \\
    AutoCorr $\downarrow$ & \pmc{0.3477}{0.1678} & \pmc{0.2545}{0.1173} & \pmcb{0.1981}{0.0583} & \pmc{0.1698}{0.0510} & \pmcb{0.1535}{0.0571} & \pmc{0.2291}{0.0094} & \pmcb{0.2194}{0.0620} \\
    D-score $\downarrow$ & \pmc{0.1805}{0.0076} & \pmcb{0.2445}{0.0202} & \pmc{0.4601}{0.0100} & \pmcb{0.2554}{0.0300} & \pmc{0.4533}{0.0068} & \pmcb{0.2208}{0.0191} & \pmc{0.4504}{0.0086} \\
    P-score $\downarrow$ & \pmc{0.0388}{0.0002} & \pmcb{0.0390}{0.0003} & \pmc{0.0622}{0.0009} & \pmcb{0.0391}{0.0003} & \pmc{0.0596}{0.0007} & \pmcb{0.0396}{0.0006} & \pmc{0.0603}{0.0005} \\
    \bottomrule
  \end{tabular}%
  }
\end{table}



==> tables/rberg_curr_pd.tex <==
\begin{table*}[t]
  \centering
  \small
  \renewcommand{\arraystretch}{1.0}
  \setlength{\tabcolsep}{3pt}
  \caption{\textbf{rBerg}: progressive distillation from a directly trained vs a curriculum-trained Sig-DEG (10) (mean $\pm$ standard deviation over 10 sampling runs). Train: total training time, including validation and the training of the parents (direct 4.83\,h, curriculum 4.46\,h). Bold marks the best in each group.}
  \label{tab:rberg_curr_pd}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{rcccccc}
    \toprule
    Method & Hist. $\downarrow$ & CrossCorr $\downarrow$ & AutoCorr $\downarrow$ & D-score $\downarrow$ & P-score $\downarrow$ & Train (h) $\downarrow$ \\
    \midrule
    Sig-DEG (5), PD $10\to5$, direct parent & \pmcb{0.0316}{0.0009} & \pmc{0.1101}{0.0140} & \pmc{0.1763}{0.0401} & \pmc{0.2670}{0.0164} & \pmcb{0.0571}{0.0002} & $5.49$ \\
    Sig-DEG (5), PD $10\to5$, curriculum parent & \pmc{0.0324}{0.0006} & \pmcb{0.1063}{0.0160} & \pmcb{0.1689}{0.0460} & \pmcb{0.2345}{0.0074} & \pmc{0.0572}{0.0002} & \numb{5.12} \\
    \midrule
    Sig-DEG (2), PD $10\to2$, direct parent & \pmc{0.0345}{0.0007} & \pmc{0.0994}{0.0239} & \pmc{0.1812}{0.0475} & \pmc{0.2524}{0.0086} & \pmcb{0.0570}{0.0002} & $5.50$ \\
    Sig-DEG (2), PD $10\to2$, curriculum parent & \pmcb{0.0336}{0.0009} & \pmcb{0.0803}{0.0129} & \pmcb{0.1371}{0.0325} & \pmcb{0.2519}{0.0165} & \pmcb{0.0570}{0.0001} & \numb{5.13} \\
    \midrule
    Sig-DEG (1), PD $10\to5\to1$, direct parent & \pmcb{0.0418}{0.0008} & \pmcb{0.0627}{0.0169} & \pmcb{0.0925}{0.0357} & \pmc{0.2916}{0.0191} & \pmc{0.0575}{0.0004} & $6.14$ \\
    Sig-DEG (1), PD $10\to5\to1$, curriculum parent & \pmc{0.0462}{0.0010} & \pmc{0.0737}{0.0148} & \pmc{0.1241}{0.0387} & \pmc{0.2493}{0.0059} & \pmc{0.0574}{0.0003} & $5.77$ \\
    Sig-DEG (1), PD $10\to2\to1$, direct parent & \pmc{0.0481}{0.0007} & \pmc{0.0727}{0.0217} & \pmc{0.1256}{0.0478} & \pmc{0.2646}{0.0076} & \pmc{0.0573}{0.0002} & $6.12$ \\
    Sig-DEG (1), PD $10\to2\to1$, curriculum parent & \pmc{0.0441}{0.0006} & \pmc{0.0778}{0.0204} & \pmc{0.1339}{0.0452} & \pmcb{0.2439}{0.0099} & \pmcb{0.0572}{0.0002} & \numb{5.75} \\
    \bottomrule
  \end{tabular}
  }
\end{table*}



==> tables/rberg_curriculum.tex <==
\begin{table*}[t]
  \normalcolor
  \centering
  \small
  \renewcommand{\arraystretch}{1.0}
  \setlength{\tabcolsep}{3pt}
  \caption{\textbf{rBerg}: direct training on the full 1000-step teacher mesh vs.\ the resolution curriculum ($125 \to 250 \to 500 \to 1000$ steps; $250 \to 500 \to 1000$ at 10 and 2 steps), at the same number of sampling steps (mean $\pm$ standard deviation over 10 sampling runs). The curriculum checkpoint is selected within the final rung; Train: total training time, including validation (Appendix~\ref{app:timing}).}
  \label{tab:rberg_curriculum}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{rcccccc}
    \toprule
    Method & Hist. $\downarrow$ & CrossCorr $\downarrow$ & AutoCorr $\downarrow$ & D-score $\downarrow$ & P-score $\downarrow$ & Train (h) $\downarrow$ \\
    \midrule
    Sig-DEG (10) & \pmcb{0.0323}{0.0005} & \pmc{0.1191}{0.0095} & \pmcb{0.2058}{0.0341} & \pmcb{0.2446}{0.0150} & \pmc{0.0575}{0.0007} & $4.83$ \\
    Sig-DEG (10) w/ Curriculum & \pmc{0.0332}{0.0010} & \pmcb{0.1148}{0.0116} & \pmc{0.2070}{0.0380} & \pmc{0.2489}{0.0169} & \pmcb{0.0572}{0.0002} & \numb{4.46} \\
    \midrule
    Sig-DEG (5) & \pmc{0.0348}{0.0010} & \pmc{0.1147}{0.0124} & \pmc{0.1943}{0.0334} & \pmc{0.2557}{0.0128} & \pmc{0.0578}{0.0004} & $6.24$ \\
    Sig-DEG (5) w/ Curriculum & \pmcb{0.0347}{0.0009} & \pmcb{0.1066}{0.0143} & \pmcb{0.1767}{0.0391} & \pmcb{0.2536}{0.0130} & \pmcb{0.0575}{0.0004} & \numb{4.98} \\
    \midrule
    Sig-DEG (2) & \pmc{0.0384}{0.0008} & \pmcb{0.1295}{0.0088} & \pmcb{0.2375}{0.0292} & \pmc{0.2669}{0.0353} & \pmcb{0.0573}{0.0006} & $11.59$ \\
    Sig-DEG (2) w/ Curriculum & \pmcb{0.0338}{0.0011} & \pmc{0.1342}{0.0065} & \pmc{0.2529}{0.0188} & \pmcb{0.2432}{0.0181} & \pmcb{0.0573}{0.0002} & \numb{7.59} \\
    \midrule
    Sig-DEG (1) & \pmcb{0.0467}{0.0008} & \pmcb{0.0731}{0.0184} & \pmcb{0.1415}{0.0437} & \pmcb{0.2191}{0.0134} & \pmcb{0.0575}{0.0004} & $13.07$ \\
    Sig-DEG (1) w/ Curriculum & \pmc{0.0504}{0.0008} & \pmc{0.1154}{0.0152} & \pmc{0.2101}{0.0351} & \pmc{0.2519}{0.0100} & \pmcb{0.0575}{0.0004} & \numb{10.73} \\
    \bottomrule
  \end{tabular}
  }
\end{table*}



==> tables/rberg_pd.tex <==
\begin{table*}[t]
  \normalcolor
  \centering
  \small
  \renewcommand{\arraystretch}{1.0}
  \setlength{\tabcolsep}{3pt}
  \caption{\textbf{rBerg}: direct training vs.\ progressive distillation (PD); $a\to b$ distils an $a$-step model into a $b$-step one (mean $\pm$ standard deviation over 10 sampling runs). Train: total training time, including validation and, for PD, the training of its parents (Sig-DEG (10): 4.83\,h).}
  \label{tab:rberg_pd}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{rcccccc}
    \toprule
    Method & Hist. $\downarrow$ & CrossCorr $\downarrow$ & AutoCorr $\downarrow$ & D-score $\downarrow$ & P-score $\downarrow$ & Train (h) $\downarrow$ \\
    \midrule
    Sig-DEG (5) & \pmc{0.0348}{0.0010} & \pmc{0.1147}{0.0124} & \pmc{0.1943}{0.0334} & \pmcb{0.2557}{0.0128} & \pmc{0.0578}{0.0004} & $6.24$ \\
    Sig-DEG (5), PD $10\to5$ & \pmcb{0.0316}{0.0009} & \pmcb{0.1101}{0.0140} & \pmcb{0.1763}{0.0401} & \pmc{0.2670}{0.0164} & \pmcb{0.0571}{0.0002} & \numb{5.49} \\
    \midrule
    Sig-DEG (2) & \pmc{0.0384}{0.0008} & \pmc{0.1295}{0.0088} & \pmc{0.2375}{0.0292} & \pmc{0.2669}{0.0353} & \pmc{0.0573}{0.0006} & $11.59$ \\
    Sig-DEG (2), PD $10\to2$ & \pmcb{0.0345}{0.0007} & \pmcb{0.0994}{0.0239} & \pmcb{0.1812}{0.0475} & \pmcb{0.2524}{0.0086} & \pmcb{0.0570}{0.0002} & \numb{5.50} \\
    \midrule
    Sig-DEG (1) & \pmc{0.0467}{0.0008} & \pmc{0.0731}{0.0184} & \pmc{0.1415}{0.0437} & \pmcb{0.2191}{0.0134} & \pmc{0.0575}{0.0004} & $13.07$ \\
    Sig-DEG (1), PD $10\to5\to1$ & \pmcb{0.0418}{0.0008} & \pmcb{0.0627}{0.0169} & \pmcb{0.0925}{0.0357} & \pmc{0.2916}{0.0191} & \pmc{0.0575}{0.0004} & $6.14$ \\
    Sig-DEG (1), PD $10\to2\to1$ & \pmc{0.0481}{0.0007} & \pmc{0.0727}{0.0217} & \pmc{0.1256}{0.0478} & \pmc{0.2646}{0.0076} & \pmc{0.0573}{0.0002} & \numb{6.12} \\
    Sig-DEG (1), PD $5\to1$ & \pmc{0.0438}{0.0010} & \pmc{0.0895}{0.0235} & \pmc{0.1511}{0.0503} & \pmc{0.2641}{0.0157} & \pmc{0.0578}{0.0005} & $6.89$ \\
    Sig-DEG (1), PD $2\to1$ & \pmc{0.0451}{0.0012} & \pmc{0.1179}{0.0114} & \pmc{0.2051}{0.0355} & \pmc{0.2505}{0.0199} & \pmcb{0.0571}{0.0002} & $12.22$ \\
    \bottomrule
  \end{tabular}
  }
\end{table*}


